Wideband Full-Duplex Wireless via Frequency-Domain Equalization: Design and Experimentation

Full-duplex (FD) wireless can significantly enhance spectrum efficiency but requires tremendous amount of self-interference (SI) cancellation. Recent advances in the RFIC community enabled wideband RF SI cancellation (SIC) in integrated circuits (ICs) via frequency-domain equalization (FDE), where RF filters channelize the SI signal path. Unlike other FD implementations, that mostly rely on delay lines, FDE-based cancellers can be realized in small-form-factor devices. However, the fundamental limits and higher layer challenges associated with these cancellers were not explored yet. Therefore, and in order to support the integration with a software-defined radio (SDR) and to facilitate experimentation in a testbed with several nodes, we design and implement an FDE-based RF canceller on a printed circuit board (PCB). We derive and experimentally validate the PCB canceller model and present a canceller configuration scheme based on an optimization problem. We then extensively evaluate the performance of the FDE-based FD radio in the SDR testbed. Experiments show that it achieves 95dB overall SIC (52dB from RF SIC) across 20MHz bandwidth, and an average link-level FD gain of 1.87x. We also conduct experiments in: (i) uplink-downlink networks with inter-user interference, and (ii) heterogeneous networks with half-duplex and FD users. The experimental FD gains in the two types of networks confirm previous analytical results. They depend on the users' SNR values and the number of FD users, and are 1.14x-1.25x and 1.25x-1.73x, respectively. Finally, we numerically evaluate and compare the RFIC and PCB implementations and study various design tradeoffs.

==> tex/algo.tex <==
$\OptProblem$ in Section~\ref{sec:background} indicates that given the RF canceller design, optimal canceller configuration is required to achieve the best RF SIC performance.
% In addition, two realistic models, $\ICTF(f_k)$ {\eqref{eq:rfic-tf}} and $\PCBTF(f_k)$ {\eqref{eq:pcb-tf}} are presented for our RFIC and PCB canceller implementations.
In this section, we present the optimization of the FDE-based RF canceller configuration based on realistic canceller models presented in Section~\ref{sec:impl}. We also derive a closed-form, near-optimal RFIC canceller configuration with $1$ FDE tap and under an ideal antenna interface. We also show that our proposed canceller configuration optimization outperforms the previously proposed iterative configuration algorithm.

% Based on the practical FDE-based RF canceller models described in Section~\ref{sec:impl}, efficient algorithms are required to optimize the configuration for each FDE tap, $\ICPCBTapTF{i}(f_k)$, to best emulate the antenna interface response, $\AntTF(f_k)$. However, there are two main challenges: (i) the real-world antenna response is non-ideal and experience high variance, and (ii) it is difficult to main analytical tractability when optimizing the joint response of multiple non-convex, complex functions.

%%
\subsection{Optimization of Canceller Configuration}
\label{ssec:algo-opt}
We present a general optimization framework that jointly optimizes all the FDE taps in the FDE-based cancellers. Although our implemented RFIC and PCB cancellers have only two FDE taps, both their models and the optimization of canceller configuration can be easily extended to the case with a larger number of FDE taps. The inputs to the FDE-based canceller configuration optimization are: (i) the RFIC or PCB canceller model with given number of FDE taps, $\NumTap$, (ii) the antenna interface response, $\AntTF(f_k)$, and the desired RF SIC bandwidth $\{f_k\}$. Then, the optimized canceller configuration are obtained by respectively solving the optimization problems $\OptProblemIC$ or $\OptProblemPCB$, in which $\ICTF(f_k)$ is given by {\eqref{eq:rfic-tf}} and $\PCBTF(f_k)$ is given by {\eqref{eq:pcb-tf-calibrated}}.
%%
\begin{align*}
\OptProblemIC\ \min: &\ \littlesum_{k=1}^{\NumChnl} \NormTwo{\ICResTF(f_k)} = \littlesum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \ICTF(f_k) }^2 \\
\textrm{s.t.:} &\ \ICTapAmp{i} \in [\ICTapAmpMin, \ICTapAmpMax],\ \ICTapPhase{i} \in [-\pi, \pi], \\
&\ \ICTapCF{i} \in [\ICTapCFMin, \ICTapCFMax],\ \ICTapQF{i} \in [\ICTapQFMin, \ICTapQFMax],\ \forall i.
\end{align*}
%%
\begin{align*}
\OptProblemPCB\ \min: &\ \littlesum_{k=1}^{\NumChnl} \NormTwo{\PCBResTF(f_k)} = \littlesum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \PCBTF(f_k) }^2 \\
\textrm{s.t.:} &\ \PCBTapAmp{i} \in [\PCBTapAmpMin, \PCBTapAmpMax],\ \PCBTapPhase{i} \in [-\pi, \pi], \\
&\ \PCBTapCFCap{i} \in [\PCBTapCFCapMin, \PCBTapCFCapMax],\ \PCBTapQFCap{i} \in [\PCBTapQFCapMin, \PCBTapQFCapMax],\ \forall i.
\end{align*}
%%

Note that the objectives of $\OptProblemIC$ and $\OptProblemPCB$ are non-convex and non-linear due to the specific forms of the configuration parameters such as (i) the higher-order terms introduced by $f_k$ in the canceller models (see {\eqref{eq:rfic-tf}} and {\eqref{eq:pcb-tf-calibrated}}), and (ii) non-linear, non-convex trigonometric terms introduced by the phase controls, $\ICTapPhase{i}$ and $\PCBTapPhase{i}$. Moreover, the non-ideal, time-varying antenna interface, $\AntTF(f_k)$, makes the optimization problem more challenging.
% Even for the RFIC canceller model {\eqref{eq:rfic-tf}} using $2^{\rm nd}$-order BPFs with an ideal antenna interface response,
In general, it is difficult to maintain analytical tractability of $\OptProblemIC$ or $\OptProblemPCB$. Therefore, a non-linear optimization solver is used to solve $\OptProblemIC$ and $\OptProblemPCB$, where the obtained canceller configuration may only be locally optimal (thus not globally optimal). However, in practice, it is unnecessary to obtain the globally optimal solution to $\OptProblemIC$ or $\OptProblemPCB$ as long as the local minimum achieved is sufficiently good, which we will show later in Sections~\ref{sec:eval-rfic} and~\ref{sec:eval-pcb}. In our FD radio design described in Section~\ref{sec:eval-pcb}, the optimized PCB canceller configuration can be obtained in less than $\SI{10}{ms}$ via a non-optimized solver.
% The conventional RF canceller~\cite{fd_demo_mobihoc16} which can only emulate the antenna interface response, $\AntTF(f_k)$, at a single frequency point, the key idea here is to use all the $\NumTap$ filter taps to jointly emulate the $\AntTF(f)$ \emph{across the desired bandwidth} $\BW = [f_1,f_\NumChnl]$.
% Essentially, solving optimizations $\OptProblemIC$ and $\OptProblemPCB$ allows the FDE-based cancellers to match with $\AntTF(f)$ not only in both amplitude and phase across the desired bandwidth, but more importantly, with the slope of the amplitude and the slope of phase (i.e., group delay).

%%
% \noindent\textbf{Optimization Algorithm}:
% \begin{enumerate}[topsep=0pt,leftmargin=*]
% %
% \item[1.]
% Given the number of FDE taps, $\NumTap$, desired RF SIC bandwidth $\BW = [f_1,f_\NumChnl]$, and the antenna interface response, $\AntTF(f_k)$;
% %
% \item[2.]
% Solve the following optimization problem $\OptProblemICPCB$ with a given RF canceller model using a nonlinear optimization solver:
% %
% %%
% \begin{align*}
% \OptProblemICPCB\ \min &\ \sum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \ICPCBTF(f_k) }^2 \\
% \textrm{s.t.} &\ \ICTF(f_k)\ \textrm{in}\ {\eqref{eq:rfic-tf}}\ \textrm{with variables}\ \{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\},\ \forall i,\ \textrm{or} \\
% &\ \PCBTF(f_k)\ \textrm{in}\ {\eqref{eq:pcb-tf-calibrated}}\ \textrm{with variables}\ \{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\},\ \forall i.\ \Box
% \end{align*}
% %%
% \end{enumerate}
%%


%% Joint optimization
% \begin{algorithm}[!h]
% \caption{Joint Optimization for the FDE Canceller}
% \label{algo:opt-joint}
% \begin{algorithmic}[1]
% % input
% \State
% Input: The number of FDE taps, $\NumTap$, the desired RF SIC bandwidth, $f_k \in [f_1,\cdots,f_K]$, and the antenna interface response, $\SIChnlTF(f_k)$,
% % solve opt
% \State
% Solve the following optimization problem using a gradient descent method:
% \begin{align}
% \min:\ & \littlesum_{k=1}^{K} \NormTwo{ \SIChnlTF(f_k) - \littlesum_{i=1}^{N} \ICPCBTapTF{i}(f_k) }^2 \nonumber \\
% \textrm{subject to}:\
% & \textrm{Variable tuning range}, \nonumber
% \end{align}
% % return
% \State
% Return the filter tap configuration.
% \end{algorithmic}
% \normalsize
% \end{algorithm}
%%


%%
%%
% \subsection{RFIC Canceller with One FDE Tap}
% \label{ssec:algo-example}
% Although it is difficult to maintain analytical tractability of $\OptProblemIC$ or $\OptProblemPCB$, if we assume that the antenna interface has an ideal response with constant amplitude of $A_{\rm SI} = |\AntTF(f_k)|$ and a constant group delay of $\tau_{\rm SI}$ (e,g., $\AntTF(f_k) = A_{\rm SI} e^{-j2\pi f_k\tau_{\rm SI}}$)\footnote{This is a reasonable assumption from our measurements (e.g., see $\AntTF(f_k)$ in Fig.~\ref{fig:exp-usrp-algo}).}, a closed-form near-optimal\footnote{This configuration is not truly optimal since approximations are applied.} configuration can be derived for the RFIC canceller with $1$ FDE tap. As we will show below, the results in this case also reveal interesting trade-offs between the amount of RF SIC that can be achieved and the desired RF SIC bandwidth. 

% We drop the subscript $i$ and superscript $\textrm{I}$ below for brevity. Let $P(f_k) := \QF{} (\CFNoidx/f_k-f_k/\CFNoidx)$, the frequency response of the RFIC canceller {\eqref{eq:rfic-tf}} with $1$ FDE tap is given by
% %%
% \begin{align}
% \label{eq:rfic-tf-expand}
% \TF{}(f_k) & = \Amp{} \cdot \frac{ 1 + jP(f_k) }{1+P^2(f_k)} \left(  \cos{\Phase{}} - j\sin{\Phase{}} \right) \nonumber \\
% & = \Amp{} \cdot \frac{(\cos{\Phase{}} + P(f_k)\sin{\Phase{}}) + j(-\sin{\Phase{}} + P(f_k)\cos{\Phase{}})}{1+P^2(f_k)} \nonumber \\
% & = \Amp{} \cdot (1+P^2(f_k))^{-1/2} \cdot e^{-j(\Phase{} - \tan^{-1}P(f_k))},
% \end{align}
% %%
% where the last step comes from the fact that
% %%
% \begin{align*}
% & \quad \left( \cos{\Phase{}} + P(f_k)\sin{\Phase{}} \right) + j \left( -\sin{\Phase{}} + P(f_k)\cos{\Phase{}} \right) \\
% & = (1+P^2(f_k))^{1/2} \cdot e^{-j(\Phase{}-\tan^{-1}P(f_k))}
% \end{align*}
% %%
% For $|f_k-\CFNoidx| \ll \CFNoidx$, it holds that $P(f_k) \approx -2\QF{}(f_k-\CFNoidx)/\CFNoidx \ll 1$. Applying the approximations $(1+x^2)^{-1/2} \approx (1-x^2/2)$ and $\tan^{-1}x \approx x$ as $x \to 0$ to {\eqref{eq:rfic-tf-expand}} yields $\TF{}(f_k) \approx \TFApprox{}(f_k) := \widetilde{\Amp{}}(f_k) e^{-j\widetilde{\ICTapPhase{}}(f_k)}$,
% where $\widetilde{\Amp{}}(f_k) := \Amp{} ( 1-P^2(f_k)/2 )$ and $\widetilde{\Phase{}}(f_k) := \Phase{}-P(f_k)$. Then, the optimal configuration of the RFIC canceller with one FDE tap can be obtained by solving $\OptProblemIC$,
% %%
% \begin{align}
% \label{eq:example-opt-obj}
% & \min:\ \littlesum_{k=1}^{K} \NormTwo{ \AntTF(f_k) - \TFApprox{}(f_k) }^2 \\
% & \textrm{s.t.:}\ \Amp{}>0,\ \Phase{} \in [-\pi, \pi],\ \CFNoidx >0,\ \QF{} > 0.
% \end{align}
% %%
% From basic trigonometric equations, we have for $\forall f_k$,
% %%
% \begin{align*}
% & | \AntTF(f_k) - \TFApprox{}(f_k) |^2 = | A_{\rm SI} e^{-j2\pi f_k \tau_{\rm SI}} - \widetilde{\Amp{}}(f_k) e^{-j\widetilde{\Phase{}}(f_k)} |^2 \\
% & \quad = (A_{\rm SI})^2 + (\widetilde{\Amp{}}(f_k))^2 - 2A_{\rm SI}\widetilde{\Amp{}}(f_k) \cos{(2\pi f_k \tau_{\rm SI} - \widetilde{\Phase{}}(f_k))}
% \end{align*}
% %%
% Using approximation $P(f_k) \approx -2\QF{}(f_k-\CFNoidx)/\CFNoidx$ yields
% %%
% \begin{align*}
% \widetilde{\Phase{}}(f_k) = \Phase{} - P(f_k) \approx \Phase{} + 2\QF{}(f_k-\CFNoidx)/\CFNoidx.
% \end{align*}
% %%
% By setting $\Phase{} = 2\pi\CFNoidx\tau_{\rm SI}\ (\textrm{mod}\ 2\pi)$ and $\QF{} = \pi\CFNoidx\tau_{\rm SI}$, we have $\widetilde{\Phase{}}(f_k) = 2\pi f_k \tau_{\rm SI},\ \forall k$. Therefore, {\eqref{eq:example-opt-obj}} becomes
% %%
% \begin{align}
% \label{eq:example-opt-obj-approx}
% \min:\ \littlesum_{k=1}^{K} \NormTwo{ \Amp{\textrm{SI}} - \Amp{} ( 1-2\pi^2\tau_{\rm SI}^2 (f_k-\CFNoidx)^2 ) }^2,
% \end{align}
% %%
% which is a quadratic function with respect to the FDE tap amplitude, $\Amp{}$, whose optimal value is given by
% %%
% \begin{align}
% \label{eq:example-opt-obj-approx-amp}
% \Amp{} = \Amp{\textrm{SI}} \cdot \left(\littlesum_{k=1}^{K} \gamma_k\right) \big/ \left(\littlesum_{k=1}^{K} \gamma_k^2\right),\ \gamma_k := 1-2\pi^2\tau_{\rm SI}^2 (f_k-\CFNoidx)^2.
% \end{align}
% %%
% Therefore, the near-optimal configuration of the FDE tap given its center frequency $\CFNoidx$, which can be selected as the center frequency of the desired SIC bandwidth (i.e., $\CFNoidx = f_{\NumChnl/2}$), is given by
% %%
% \begin{align}
% \Amp{}\ \textrm{in}\ {\eqref{eq:example-opt-obj-approx-amp}},\ \Phase{} = 2\pi f_c \tau_{\rm SI}\ (\textrm{mod}\ 2\pi),\ \textrm{and}\ \QF{} = \pi \CFNoidx \tau_{\rm SI}.
% \end{align}
% %%
% {\eqref{eq:example-opt-obj-approx}} and {\eqref{eq:example-opt-obj-approx-amp}} show that as the desired RF SIC bandwidth increases (i.e., $|f_k-\CFNoidx|$ increases for given values of $\CFNoidx$ and $K$), the residual SI power level {\eqref{eq:example-opt-obj-approx}} increases, resulting in degraded RF SIC performance.


%%
%%
% \subsection{Iterative Configuration Algorithm}
% \label{ssec:algo-iter}
% In~\cite{Zhou_WBSIC_JSSC15}, an iterative configuration algorithm was proposed to find the RFIC canceller configuration. Specifically, the first FDE tap $\ICTapTF{1}(f_k)$ is optimized to match with the amplitude and phase and their slopes of the antenna interface at a given cancellation frequency $f_{\textrm{canc}, 1}$. Then, the second FDE tap $\ICTapTF{2}(f_k)$ is optimized to match with those of the residual SI channel ($\AntTF(f_k) - \ICTapTF{2}(f_k)$), at a different cancellation frequency $f_{\textrm{canc}, 2}$. We generalize this iterative configuration algorithm based on both the RFIC and PCB canceller models as the process below.
% %%
% \begin{enumerate}[topsep=0pt, leftmargin=*]
% \item[1.]
% Given the FDE-based canceller model with $\NumTap$ FDE taps, the desired RF SIC bandwidth $\{f_k\}$, the antenna interface response, $\AntTF(f_k)$. Select a sequence of cancellation frequencies, $\{f_{\textrm{canc}, i}\}_{i=1}^{\NumTap}$, and set the initial residual SI channel as $\ResTapTF{0}(f_k) = \AntTF(f_k)$;
% %
% \item[2.]
% For $\forall i$, solve for the configuration of the $i^{\rm th}$ FDE tap such that $\ResTapTF{i-1}(f_k)$ and $\RFCancTapTF{i}(f_k)$ are equal in amplitude, phase, and the slopes of amplitude and phase, at cancellation frequency $f_{\textrm{canc},i}$. Update the residual SI channel by setting $\ResTapTF{i}(f_k) = \ResTapTF{i-1}(f_k) - \RFCancTapTF{i}(f_k)$.
% \end{enumerate}
% %%
% For the RFIC canceller {\eqref{eq:rfic-tf}}, closed-form solutions of $\{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\}$ when solving step 2 can be obtained by simple analysis~\cite{Zhou_WBSIC_JSSC15}. For the PCB canceller {\eqref{eq:pcb-tf-calibrated}}, $\{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\}$ can be obtained easily by solving step 2 numerically.

% In Section~\ref{ssec:eval-rfic-compare}, we compare the RFIC canceller performance under both the iterative configuration algorithm and with the optimized canceller configuration. As we will show, the iterative configuration algorithm performs poorly since it does not jointly optimize all the FDE taps. More importantly, the introduction of a new $i^{\rm th}$ FDE tap, $\RFCancTapTF{i}(f_k)$, will adversely affect the residual SI channel $\ResTapTF{i-1}(f_k)$ from the previous iteration (see step 2) at its cancellation frequency $f_{\textrm{canc}, i-1}$. Despite one strength which is its low complexity, it also remains unclear how the cancellation frequencies, $f_{\textrm{canc,} i}$, can be optimally selected for the FDE taps.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/eval_rfic.tex <==
Our RFIC canceller implementation in~\cite{Zhou_WBSIC_JSSC15} has only $2$ FDE taps and achieves an average $\SI{40}{dB}$ RF SIC across $\SI{27}{MHz}$ bandwidth. Recall that the model {\eqref{eq:rfic-tf}} (see Section~\ref{ssec:impl-rfic}) accurately captures the responses of the RFIC canceller~\cite{ghaffari2011tunable,Zhou_WBSIC_JSSC15} and can be scaled up to a larger number of FDE taps. Therefore, we numerically evaluate the performance of the RFIC canceller using the model {\eqref{eq:rfic-tf}}, and the optimized canceller configuration described in Section~\ref{ssec:algo-opt}. Throughout our evaluation, we use a \emph{real, practical} antenna interface response, $\AntTF(f_k)$, measured using a $698$-$\SI{960}{MHz}$ swivel blade antenna with a coaxial circulator with operating frequency range $860$-$\SI{960}{MHz}$ in a lab environment.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-20mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_20mhz.eps}
}
% \hspace{-12pt}
\subfloat{
\label{fig:eval-rfic-bw-40mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_40mhz.eps}
}
\\ \vspace{-\baselineskip}
%%
% \subfloat{
% \label{fig:eval-rfic-bw-60mhz}
% \includegraphics[width=0.45\columnwidth]{./figs/sim/sim_rfic_bw_60mhz.eps}
% }
% \hspace{-12pt}
\subfloat{
\label{fig:eval-rfic-bw-80mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_80mhz.eps}
}
\vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface and with the RFIC canceller {\eqref{eq:rfic-tf}} with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{20,40,80\}\thinspace\SI{}{MHz}$.}
\label{fig:eval-rfic}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\subsection{The Ideal Case}
To evaluate and validate the concept of FDE, we first simulate the RF SIC achieved by the RFIC canceller with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{20,40,80\}\thinspace\SI{}{MHz}$. We only report the RF SIC performance with up to $\NumTap=4$ FDE taps since, as we show below, this case can achieve sufficient RF SIC performance up to $\SI{80}{MHz}$ bandwidth.\footnote{We select $\{20,40,80\}\thinspace\SI{}{MHz}$ desired RF SIC bandwidth since: (i) these are the standard WiFi bandwidths, and (ii) the circulator has an operating frequency range of $\SI{100}{MHz}$.} Fig.~\ref{fig:eval-rfic} shows the TX/RX isolation (defined in Section~\ref{sec:background}) without and with the RFIC canceller, where the isolation at the antenna interface $|\AntTF(f_k)| \approx -\SI{20}{dB}$. The optimized RFIC canceller configurations are obtained by solving the optimization problem $\OptProblemIC$ with the following constraints: $\forall i$, $\ICTapAmp{i} \in [-40, -10]\thinspace\SI{}{dB}$, $\ICTapPhase{i} \in [-\pi, \pi]$, $\ICTapCF{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\ICTapQF{i} \in [1, 50]$. These constraints are practically selected and can be easily realized in an RFIC implementation.

Fig.~\ref{fig:eval-rfic} shows that (i) a larger number of FDE taps can significantly enhance the RF SIC bandwidth, and (ii) under the same desired RF SIC bandwidth, a larger number of FDE taps results in better average RF SIC performance. With only $2$ FDE taps, the RFIC canceller achieves an average $\SI{58}{dB}$ RF SIC with $\SI{20}{MHz}$ bandwidth, but this value decreases to only $\SI{47}{dB}$ with $\SI{40}{MHz}$ bandwidth. With $4$ FDE taps, the RFIC canceller achieves an average amount of more than $\SI{56}{dB}$ RF SIC for all considered RF SIC bandwidth up to $\SI{80}{MHz}$.
% Fig.~\ref{fig:theory-sim-varying-bw} also shows that the RF SIC performance does not degrade for $N=2,3$ FDE taps when the desired SIC bandwidth is increased, ilustrating that $2$ or $3$ ideal FDE taps are robust to medium SIC bandwidth requirements.
Fig.~\ref{fig:eval-rfic} also shows that in some scenarios, adding more FDE taps does not help increase the RF SIC performance. For example, an RFIC canceller with $3$ FDE taps already achieves more than $\SI{70}{dB}$ RF SIC with $\SI{20}{MHz}$ bandwidth, and adding a fourth FDE tap only introduces minimal performance improvement. Note that we constrain the center frequency of the $2^{\rm nd}$-order BPFs in {\eqref{eq:rfic-tf}} to be within a $\SI{50}{MHz}$ range, and performance improvement is expected by relaxing this constraint.


%%
\subsection{Adding Practical Quantization Constraints}
In practice, the values of $\{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\}$ can not be arbitrarily selected from a continuous range. Instead, they are often restricted to discrete values given the resolution of the corresponding hardware components. We evaluate the effect of such practical quantization constraints with the following settings. The amplitude $\ICTapAmp{i}$ has a $\SI{0.25}{dB}$ resolution within range $[-40, -10]\thinspace\SI{}{dB}$. For $\ICTapPhase{i} \in [-\pi, \pi]$, $\ICTapCF{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\ICTapQF{i} \in [1, 50]$, an $8$-bit resolution constraint is introduced, which is equivalent to $2^8=256$ discrete values spaced equally in the given range. The RFIC canceller configurations with quantization constraints are obtained by rounding the configurations returned by $\OptProblemIC$ to their closest quantized values.

Fig.~\ref{fig:eval-rfic-quantized} presents the TX/RX isolation without and with the RFIC canceller with $\NumTap \in \{1,2,3,4\}$ and $\{40, 80\}\thinspace\SI{}{MHz}$ desired RF SIC bandwidth, under practical quantization constraints. The results for $20\thinspace\SI{}{MHz}$ desired RF SIC bandwidth are similar and thus omitted here. Comparing Fig.~\ref{fig:eval-rfic-quantized} with Fig.~\ref{fig:eval-rfic} shows that adding practical quantization constraints slightly reduces the amount of RF SIC achieved across the desired bandwidth. In particular, the effect of quantized configurations is the most significant for the case with $4$ FDE taps. This is because that as more FDE taps are available, more flexibility exists due to a larger number of variables that can be controlled. As a result, the RF SIC performance becomes more sensitive to the coupling between individual FDE tap responses after quantization. However, as Fig.~\ref{fig:eval-rfic-quantized} suggests, even under practical quantization constraints, an RFIC canceller with $4$ FDE taps can achieve an average $\SI{50}{dB}$ RF SIC across up to $\SI{80}{MHz}$ desired bandwidth. In addition, by relaxing the quantization constraints (e.g., through using components with higher resolutions), performance improvement is expected.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-quantized-bw-40mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_40mhz_quantized.eps}}
% \hspace{-10pt} \hfill
\subfloat{
\label{fig:eval-rfic-quantized-bw-80mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_80mhz_quantized.eps}
}
\vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface and with the RFIC canceller {\eqref{eq:rfic-tf}} with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{40,80\}\thinspace\SI{}{MHz}$, under practical quantization constraints}
\label{fig:eval-rfic-quantized}
\vspace{-\baselineskip}
\end{figure}
%%


%%
\subsection{Comparison with the Iterative Algorithm}
\label{ssec:eval-rfic-compare}
We now compare the RFIC canceller performance under the iterative configuration algorithm and with the optimized canceller configuration, with the same practical quantization constraints as described above. As described in Section~\ref{ssec:algo-iter}, for the iterative configuration algorithm, the selection of the cancellation frequency is unclear. Therefore, we manually find the best cancellation frequencies, $\{f_{\textrm{canc},i}\}$, such the RFIC canceller performance is optimized under the iterative configuration algorithm. Moreover, we consider only $2$ FDE taps since the performance of the iterative configuration algorithm with a larger value of $\NumTap$ performs even poorly when compared with the that with the optimized canceller configuration.

Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-detail} shows the process of the iterative configuration algorithm, where $\ICTapTF{1}(f_k)$ and $\ICTapTF{2}(f_k)$ are used to match with $\AntTF(f_k)$ and $H_{\textrm{res},1}(f_k) = \AntTF(f_k)-\ICTapTF{1}(f_k)$, respectively, at the manually-optimized cancellation frequencies $\SI{896}{MHz}$ and $\SI{904}{MHz}$ indicated by the asterisks. As Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-detail} shows, the $\SI{40}{dB}$ RF SIC bandwidth is improved from $\SI{10}{MHz}$ to $\SI{16}{MHz}$ by using a second FDE tap. However, Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-compare} shows that this approach suffers from a large performance degradation when compared with the RFIC canceller performance with the optimized canceller configuration. Therefore, the optimal canceller configuration is more beneficial, which is also used to evaluate the PCB canceller performance in Section~\ref{sec:eval-pcb}.

%%
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[]{
\label{fig:eval-rfic-iter-detail}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_iter_detail.eps}
}
% \hspace{-6pt} \hfill
\subfloat[]{
\label{fig:eval-rfic-iter-compare}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_iter_compare.eps}
}
\vspace{-\baselineskip}
\caption{(a) TX/RX Isolation of the antenna interface and with the RFIC canceller after each iterative configuration step. (b) Comparison of TX/RX isolation performance under the iterative and optimal configurations.}
% where each FDE tap matches with the residual SI channel response from the previous iteration at a cancellation frequency indicated by the marker.
\label{fig:eval-rfic-iter}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/experiments_20180807.tex <==
%%
In this section, we discuss the integration of the PCB canceller described in Section~\ref{sec:impl} with an SDR testbed. Then, we present extensive experimental evaluation of the FDE-based FD radio at the node, link, and network levels.

%%%%%
%%%%%
\subsection{Implementation and Testbed}
\label{ssec:exp-testbed}

\noindent\textbf{FDE-based FD Radio and the SDR Testbed}.
Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-fd-net} depict our FDE-based FD radio design and the SDR testbed. A $698$--$\SI{960}{MHz}$ swivel blade antenna and a coaxial circulator with operating frequency range $860$--$\SI{960}{MHz}$ are used as the antenna interface. We use the NI USRP-2942 SDR with carrier frequency at $\SI{900}{MHz}$, which is the same as the operating frequency of the antenna interface and the PCB canceller with 2 FDE taps.\footnote{As mentioned in Section~\ref{ssec:impl-pcb}, our PCB canceller design can be easily extended to other operating frequencies.} The USRP has a measured noise floor of $-\SI{85}{dBm}$ at a fixed receiver gain setting.\footnote{This USRP receiver noise floor is limited by the environmental interference at around $\SI{900}{MHz}$ frequency. The USRP has a true noise floor of around $-\SI{95}{dBm}$ at the same receiver gain setting, when not connected to an antenna.}

We implemented a full OFDM-based PHY layer using NI LabVIEW on a host PC. A real-time RF bandwidth of $\BW=\SI{20}{MHz}$ is used through our experiments. The baseband complex (IQ) samples are streamed between the USRP and the host PC through a high-speed PCI-Express interface. The OFDM symbol size is 64 samples (subcarriers) with a cyclic-prefix ratio of 0.25 (16 samples). Throughout the evaluation, $\{f_k\}_{k=1}^{K=52}$ is used to represent the center frequency of the 52 non-zero subcarriers. The OFDM PHY layer supports various modulation and coding schemes (MCSs) with constellations from BPSK to 64QAM and coding rates of 1/2, 2/3, and 3/4, resulting in a highest (HD) data rate of $\SI{54}{Mbps}$.
% Unless mentioned otherwise, we cycle through all MCSs in the experiments and record the maximal achieved data rate.
The digital SIC algorithm with a highest non-linearity order of 7 is also implemented in LabVIEW to further suppress the residual SI signal after RF SIC.\footnote{The digital SIC algorithm is based on Volterra series and a least-square problem, which is similar to that presented in~\cite{bharadia2013full}. We omit the details here due to limited space.}

In total, our testbed consists of 3 FDE-based FD radios, whose performance is experimentally evaluated at the node, link, and network levels. Regular USRPs (without the PCB canceller) are also included in scenarios where additional HD users are needed.

%%
%%
\noindent\textbf{Optimized PCB Canceller Configuration}.
We implement the optimized PCB canceller configuration scheme on the host PC and the canceller is configured by a SUB-20 controller through the USB interface. To achieve computational efficiency, the PCB canceller response {\eqref{eq:pcb-tf-calibrated}} (which is independent of the environment) is pre-computed and stored. The detailed steps of the canceller configuration are as follows.
%%
\begin{enumerate}[topsep=0pt,itemsep=-3pt,leftmargin=*]
\item[1.]
Measure the real-time antenna interface response, $\AntTF(f_k)$, using a preamble (2 OFDM symbols) by dividing the received preamble by the known transmitted preamble in the frequency domain;
\item[2.]
Solve for an initial PCB canceller configuration using optimization {\OptProblemPCB} based on the measured $\AntTF(f_k)$ and the canceller model {\eqref{eq:pcb-tf-calibrated}} (see Section~\ref{ssec:impl-opt}). The returned configuration parameters are rounded to their closest possible values based on hardware resolutions (see Section~\ref{ssec:impl-pcb});
\item[3.]
Perform a finer-grained local search and record the optimal canceller configuration (usually \texttt{\char`\~}10 iterations).
\end{enumerate}
%%
In our design, the optimized PCB canceller configuration can be obtained in less than $\SI{10}{ms}$ on a regular PC with quad-core Intel i7 CPU via a non-optimized MATLAB solver.\footnote{Assuming that the canceller needs to be configured once per second, this is only a $1\%$ overhead. We note that an FPGA-based implementation can significantly improve the performance of the canceller configuration scheme and is left for future work.}

%%
%%


%%%%%
%%%%%
\subsection{Node-Level: Microbenchmarks}
\label{ssec:exp-node}

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-usrp-algo-iq}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_iq.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-usrp-algo-res}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_res.eps}
}
\vspace{-0.5\baselineskip}
\caption{(a) Real and imaginary parts of the optimized PCB canceller response, $\PCBTF(f_k)$, vs. real-time SI channel measurements, $\AntTF(f_k)$, and (b) modeled and measured RX signal power after RF SIC at $\SI{10}{dBm}$ TX power. An average $\SI{52}{dB}$ RF SIC across $\SI{20}{MHz}$ is achieved in the experiments.}
\label{fig:exp-usrp-algo}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
\noindent\textbf{Optimized PCB Canceller Response and RF SIC}.
We set up an FDE-based FD radio running the optimized PCB canceller configuration scheme and record the canceller configuration, measured $\AntTF(f_k)$, and measured residual SI power after RF SIC. The recorded canceller configuration is then used to compute the PCB canceller response using {\eqref{eq:pcb-tf-calibrated}}.

Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-iq} shows an example of the optimized PCB canceller response, $\PCBTF(f_k)$, and the measured antenna interface response, $\AntTF(f_k)$, in real and imaginary parts (or I and Q). It can be seen that $\PCBTF(f_k)$ closely matches with $\AntTF(f_k)$ with maximal amplitude and phase differences of only $\SI{0.5}{dB}$ and $\SI{2.5}{\degree}$, respectively. This confirms the accuracy of the PCB canceller model and the performance of the optimized canceller configuration. Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-res} shows the modeled (computed by subtracting the modeled canceller response from the measured $\AntTF(f_k)$) and measured RX signal power after RF SIC at $\SI{10}{dBm}$ TX power. The results show that the FDE-based FD radio achieves an average $\SI{52}{dB}$ RF SIC across $\SI{20}{MHz}$ bandwidth, from which $\SI{20}{dB}$ is obtained from the antenna interface isolation. Similar performance is observed in various experiments throughout the experimental evaluation.
% Note that the profile of RF SIC is similar to that presented in the sensitivity analysis of the FDE-based cancellers (see Section~\ref{sec:sensitivity}).

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-.5\baselineskip}
\includegraphics[width=0.7\columnwidth]{./figs/exp/exp_usrp_sic.eps}
\vspace{-0.5\baselineskip}
\caption{Power spectrum of the received signal after SIC in the RF and digital domains with $\SI{10}{dBm}$ average TX power, $\SI{20}{MHz}$ bandwidth, and $-\SI{85}{dBm}$ receiver noise floor.}
\label{fig:eval-usrp-spec-20mhz}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
%%
\noindent\textbf{Overall SIC}.
We measure the overall SIC achieved by the FDE-based FD radio including the digital SIC in the same setting as described above, and the results are presented in Fig.~\ref{fig:eval-usrp-spec-20mhz}. It can be seen that the FDE-based FD radio achieves an average $\SI{95}{dB}$ overall SIC across $\SI{20}{MHz}$, from which $\SI{52}{dB}$ and $\SI{43}{dB}$ are obtained in the RF and digital domains, respectively. Recall from Section~\ref{ssec:exp-testbed} that the USRP has noise floor of $\SI{-85}{dBm}$, the FDE-based RF radio supports a maximal average TX power of $\SI{10}{dBm}$ (where the peak TX power can go as high as $\SI{20}{dBm}$). We use TX power levels lower than or equal to $\SI{10}{dBm}$ throughout the experiments, where all the SI can be canceled to below the RX noise floor.


%%
%%
\subsection{Link-Level: SNR-PRR Relationship}
\label{ssec:exp-snr-prr-relationship}
We now evaluate the relationship between link SNR and link packet reception ratio (PRR). We setup up a link with two FDE-based FD radios at a fixed distance of 5 meters with equal TX power. We set an FD radio to operate in HD mode by turning on only its transmitter or receiver, since we would like to evaluate it performance with the existence of the PCB canceller. The following experiments are conducted for all possible MCSs and varying TX power level of the radios. In each experiment, both FD radios send a sequence of 50 OFDM streams in both HD and FD modes, each containing 20 OFDM packets with length 800 Bytes. The packets are sent over the link simultaneously in FD mode and in alternating directions in HD mode (i.e., the two radios take turns and transmit to each other).

We consider two metrics. The \emph{HD (resp.\ FD) link SNR} is measured as the ratio between the average RX signal power in both directions and the RX noise floor when both radios operate in HD (resp. FD) mode. The \emph{HD (resp.\ FD) link PRR} is computed as the fraction of packets successfully sent over the HD (resp. FD) link in each experiment. We observe from the experiments that the HD and FD link SNR and PRR values in both link directions are similar. Similar experiments and results were presented in~\cite{zhou2016basic} for HD links.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[Code rate 1/2]{
\label{fig:exp-prr-vs-snr-1-2}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_1_2.eps}
}
\hfill
\subfloat[Code rate 3/4]{
\label{fig:exp-prr-vs-snr-3-4}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link packet reception ratio (PRR) with varying HD link SNR and modulation and coding schemes (MCSs).}
\label{fig:exp-prr-vs-snr}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

Fig.~\ref{fig:exp-prr-vs-snr} shows the relationship between link PRR values and HD link SNR values with varying MCSs. The results show that with sufficient link SNR values (e.g., $\SI{8}{dB}$ for BPSK-1/2 and $\SI{28}{dB}$ for 64QAM-3/4), the FDE-based FD radio achieves a link PRR of $100\%$. With insufficient link SNR values, the average FD link PRR is $6.5\%$ lower than the HD link PRR across varying MCSs. This degradation is caused by the link SNR difference when the radios operate in HD or FD mode, which is described later in Section~\ref{ssec:exp-link}. Since packets are sent simultaneously in both directions on an FD link, this average PRR degradation is equivalent to an average FD link throughput gain of $1.87\times$ under the same MCS.


%%%%%
%%%%%
\subsection{Link-Level: SNR Difference and FD Gain}
\label{ssec:exp-link}

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-0.5\baselineskip}
\subfloat[LOS deployment and an FD radio in a hallway]{
\label{fig:exp-map-los}
\includegraphics[width=1\columnwidth]{./figs/exp/link/exp_los_setup.pdf}
} \\
\vspace{-0.5\baselineskip}
% \hspace{6pt}
\subfloat[NLOS deployment and an FD radio in a lab environment]{
\label{fig:exp-map-nlos}
\includegraphics[width=1\columnwidth]{./figs/exp/link/exp_nlos_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{(a) Line-of-sight (LOS), and (b) non-line-of-sight (NLOS) deployments, and the measured HD link SNR values (dB).}
\label{fig:exp-map}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{Experimental Setup}.
To thoroughly evaluate the link level FD throughput gain achieved by our FD radio design, we conduct experiments with two FD radios with $\SI{10}{dBm}$ TX power, one emulating a base station (BS) and one emulating a user. We consider both line-of-sight (LOS) and non-line-of-sight (NLOS) experiments as shown in Fig.~\ref{fig:exp-map}. In the LOS setting, the BS is placed at the end of a hallway and the user is moved away from the BS at stepsizes of 5 meters up to a distance of 40 meters. In the NLOS setting, the BS is placed in a lab environment with regular furniture and the user is placed at various locations (offices, labs, and corridors). The measured HD link SNR values are also included in Fig.~\ref{fig:exp-map}. Following the methodology of~\cite{bharadia2013full}, for each user location, we measure the \emph{link SNR difference}, which is defined as the absolute difference between the average HD and FD link SNR values. Throughout the experiments, link SNR values between $0$ -- $\SI{50}{dB}$ are observed.


%%
%%
\noindent\textbf{Difference in HD and FD Link SNR Values}.
Fig.~\ref{fig:exp-link-snr-loss} shows the measured link SNR difference as a function of the HD link SNR (i.e., for different user locations) in the LOS and NLOS experiments, respectively, with 64QAM-3/4 MCS. For the LOS experiments, the average link SNR difference is $\SI{0.6}{dB}$ with a standard deviation of $\SI{0.16}{dB}$. For the NLOS experiments, the average link SNR difference is $\SI{0.63}{dB}$ with a standard deviation of $\SI{0.31}{dB}$. The SNR difference has a higher variance in the NLOS experiments, due to the complicated environments (e.g., wooden desks and chairs, metal doors and bookshelves, etc.). In both cases, the link SNR difference is minimal and uncorrelated with user locations, showing the robustness of the FDE-based FD radio.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-snr-loss-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_snr_loss.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-snr-loss-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_snr_loss.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values in the (a) LOS, and (b) NLOS experiments, with $\SI{10}{dBm}$ TX power and 64QAM-3/4 MCS.}
\label{fig:exp-link-snr-loss}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{Impact of Constellations}.
Fig.~\ref{fig:exp-constellation} shows the measured link SNR difference and its CDF with varying constellations and 3/4 coding rate. It can be seen that the link SNR difference has a mean of $\SI{0.58}{dB}$ and a standard deviation of $\SI{0.4}{dB}$, both of which are uncorrelated with the constellations.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-constellation-snr-loss}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_err.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-constellation-tput-gain}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_cdf.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values with $\SI{10}{dBm}$ TX power under varying constellations: (a) mean and standard deviation, and (b) CDF.}
\label{fig:exp-constellation}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{FD Link Throughput and Gain}.
For each user location in the LOS and NLOS experiments, the HD (resp.\ FD) link throughput is measured as the highest average data rate across all MCSs achieved by the link when both nodes operate in HD (resp.\ FD) mode . The FD gain is computed as the ratio between FD and HD throughput values. Recall that the maximal HD data rate is $\SI{54}{Mbps}$, an FD link data rate of $\SI{108}{Mbps}$ can be achieved with an FD link PRR of 1.

Fig.~\ref{fig:exp-link-tput} shows the average HD and FD link throughput with varying 16QAM-3/4 and 16QAM-3/4 MCSs, where each point represents the average throughput across 1,000 packets. The results show that with sufficient link SNR (e.g., $\SI{30}{dB}$ for 64QAM-3/4 MCS), the FDE-based FD radios achieve an \emph{exact} link throughput gain of $2\times$ with an HD/FD link PRR of 1. Namely, in cases in which the data rate is limited by the MCS, enabling FD communication results in an \emph{exact} throughput gain of $2\times$. With medium link SNR values, where the link PRR less than 1, the average FD link throughput gains across different MCSs are $1.91\times$ and $1.85\times$ for the LOS and NLOS experiments, respectively.


%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-tput-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_tput_3_4.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-tput-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_tput_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link throughput in the (a) LOS, and (b) NLOS experiments, with $\SI{10}{dBm}$ TX power and 16QAM-3/4 and 64QAM-3/4 MCSs.}
\label{fig:exp-link-tput}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%
\subsection{Network-Level FD Gain}
\label{ssec:exp-net}
We now experimentally evaluate the network-level throughput gain introduced by FD-capable BS and users. The users can significanlty benefit from the FDE-based FD radio suitable for hand-held devices. We compare experimental results to the analysis (e.g.,~\cite{marasevic2017resource}) and demonstrate practical FD gain in different network settings. Specifically, we consider two types of networks as depicted in Fig.~\ref{fig:exp-net-setup}: (i) \emph{UL-DL networks} with one FD BS and two HD users with inter-user interference (IUI), and (ii) \emph{heterogeneous HD-FD networks} with HD and FD users. Due to hardware limitations, we apply a TDMA setting where each (HD or FD) user takes turn to be activated for the same period of time.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-net-setup-ul-dl}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_ul_dl/exp_ul_dl_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-two-users}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_two_users/exp_two_users_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-three-users}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_three_users/exp_three_users_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{An example experimental setup for: (a) the UL-DL networks with varying $\SNRUL$ and $\SNRDL$, (b) heterogeneous 3-node network with one FD BS and 2 FD users, and (c) heterogeneous 4-node networks with one FD BS, 2 FD users, and one HD user.}
\label{fig:exp-net-setup}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%
\subsubsection{UL-DL Networks with IUI}
\label{sssec:exp-net-ul-dl}
We first consider UL-DL networks consisting of one FD BS and two HD users (indexed 1 and 2). Without loss of generality, in this setting, user 1 transmits on the UL to the BS, and the BS transmits to user 2 on the DL (see Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}).

%%
%%
\noindent\textbf{Analytical FD gain}.
We use Shannon's capacity formula $\DataRate{}(\SNR{}) = \BW \cdot \log_{2}(1+\SNR{})$ to compute the \emph{analytical throughput} of a link under bandwidth $\BW$ and link SNR $\SNR{}$. If the BS is only HD-capable, the network throughput in a UL-DL network when the UL and DL share the channel in a TDMA manner with equal fraction of time is given by
%%
\begin{align}
\label{eq:net-ul-dl-tput-hd}
\textstyle
\DataRate{\textrm{UL-DL}}^{\textrm{HD}} = \frac{\BW}{2}\log\left(1+\SNRUL\right) + \frac{\BW}{2}\log\left(1+\SNRDL\right),
\end{align}
%%
where $\SNRUL$ and $\SNRDL$ are the UL and DL SNRs, respectively.

If the BS is FD-capable, the UL and DL can be simultaneously activated with an analytical network throughput of
%%
\begin{align}
\label{eq:net-ul-dl-tput-fd}
\textstyle
\DataRate{\textrm{UL-DL}}^{\textrm{FD}} = \BW\log\left(1+\frac{\SNRUL}{1+\XINR}\right) + \BW\log\left(1+\frac{\SNRDL}{1+\IUI}\right),
\end{align}
%%
where: (i) $\frac{\SNRDL}{1+\IUI}$ is the signal-to-interference-plus-noise ratio (SINR) at the DL HD user, and (ii) $\XINR$ is the residual self-interference-to-noise ratio (XINR) at the FD BS. We set $\XINR=1$ when computing the analytical throughput. Namely, the residual SI power is no higher than the RX noise floor (which can be achieved by the FDE-based FD radio, see Section~\ref{ssec:exp-node}). The \emph{analytical FD gain} is then defined as the ratio $\left(\DataRate{\textrm{UL-DL}}^{\textrm{FD}}/\DataRate{\textrm{UL-DL}}^{\textrm{HD}}\right)$. Note that the FD gain depends on the coupling between $\SNRUL$, $\SNRDL$, and $\IUI$, which depend on the BS/user locations, their TX power, etc. 

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[$\SNRUL=\SI{10}{dB}$]{
\label{fig::exp-net-ul-dl-gain-10db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_10db.eps}
}
\subfloat[$\SNRUL=\SI{15}{dB}$]{
\label{fig::exp-net-ul-dl-gain-15db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_15db.eps}
}
\subfloat[$\SNRUL=\SI{20}{dB}$]{
\label{fig::exp-net-ul-dl-gain-20db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_20db.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for UL-DL networks consisting of one FD BS and two HD users with varying UL and DL SNR values, and inter-user interference (IUI) levels: (a) $\SNRUL=\SI{10}{dB}$, (b) $\SNRUL=\SI{15}{dB}$, and (c) $\SNRUL=\SI{20}{dB}$. The baseline is the network throughput when the BS is HD.}
\label{fig:exp-net-ul-dl-gain}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
%%
\noindent\textbf{Experimental FD gain}.
The experimental setup is depicted in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}, where the TX power levels of the BS and user 1 are set to be $\SI{10}{dBm}$ and $\SI{-10}{dBm}$, respectively. We fix the location of the BS and consider different UL SNR values of $\SNRUL = 10/15/20\thinspace\SI{}{dB}$ by placing user 1 at three different locations. For each value of $\SNRUL$, user 2 is placed at 10 different locations, resulting in varying $\SNRDL$ and $\IUI$ values.

%% table begins
\begin{table}[!t]
\caption{Average FD Gain in UL-DL Networks with IUI.}
\label{table:exp-net-ul-dl-gain}
\vspace{-1.5\baselineskip}
\scriptsize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\begin{tabular}{|c|c|c|}
\hline
UL SNR, $\SNRUL$ & Analytical FD Gain & Experimental FD Gain \\
\hline
$\SI{10}{dB}$ & $1.30\times$ & $1.25\times$ \\
\hline
$\SI{15}{dB}$ & $1.23\times$ & $1.16\times$ \\
\hline
$\SI{20}{dB}$ & $1.22\times$ & $1.14\times$ \\
\hline
\end{tabular}
\end{center}
\vspace{-2\baselineskip}
\end{table}
%% table ends

Fig.~\ref{fig:exp-net-ul-dl-gain} shows the analytical (colored surface) and experimental (filled circles) FD gain, where the analytical gain is extracted using {\eqref{eq:net-ul-dl-tput-hd}} and {\eqref{eq:net-ul-dl-tput-fd}}, and the experimental gain is computed using the measured UL and DL throughput. It can be seen that smaller values of $\SNRUL$ and lower ratios between $\SNRDL$ and $\IUI$ lead to higher throughput gains in both analysis and experiments. The average analytical and experimental FD gains are summarized in Table~\ref{table:exp-net-ul-dl-gain}. Due to practical reasons such as the link SNR difference and its impact on link PRR (see Section~\ref{ssec:exp-snr-prr-relationship}), the experimental FD gain is $7\%$ lower than the analytical FD gain. The results confirm the analysis in~\cite{marasevic2017resource} and demonstrate the practical FD gain achieved in wideband UL-DL networks without any changes in the current network stack (i.e., only bringing FD capability to the BS). Moreover, performance improvements are expected through advanced power control and scheduling schemes.


%%%%%
%%%%%
\subsubsection{Heterogeneous 3-Node Networks}
\label{sssec:exp-net-two-users}

We consider heterogeneous HD-FD networks with 3 nodes: one FD BS and two users that can operate in either HD or FD mode (see an example experimental setup in Figs.\ref{fig:intro}\subref{fig:intro-fd-net} and~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-two-users}). All 3 nodes have the same $\SI{0}{dBm}$ TX power so that each user has symmetric UL and DL SNR values of $\SNR{i}$ ($i=1,2$).
% \footnote{To better illustrate the results, we consider symmetric UL and DL SNR values while the link SNRs are different across users. The case with asymmetric UL and DL SNR values can also be evaluated.}
We place user 1 at 5 different locations and place user 2 at 10 different locations for each location of user 1, resulting in a total number of 50 pairs of $(\SNR{1},\SNR{2})$.


%%
%%
\noindent\textbf{Analytical FD gain}.
We set the users to share the channel in a TDMA manner. The analytical network throughput in a 3-node network when zero, one, and two users are FD-capable is respectively given by
%%
\begin{align}
& \textstyle \DataRate{}^{\textrm{HD}} = \frac{\BW}{2}\log\left(1+\SNR{1}\right) + \frac{\BW}{2}\log\left(1+\SNR{2}\right), \label{eq:net-two-users-tput-hd} \\
& \textstyle \DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}} = \BW\log\left(1+\frac{\SNR{i}}{1+\XINR}\right) + \frac{\BW}{2}\log\left(1+\SNR{\bar{i}}\right),\ \label{eq:net-two-users-tput-hd-fd} \\
& \textstyle \DataRate{}^{\textrm{FD}} = \BW\log\left(1+\frac{\SNR{1}}{1+\XINR}\right) + \BW\log\left(1+\frac{\SNR{2}}{1+\XINR}\right), \label{eq:net-two-users-tput-fd}
\end{align}
%%
where $\XINR=1$ is set (similar to Section~\ref{sssec:exp-net-ul-dl}). We consider both FD gains of $\left(\DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}}/\DataRate{}^{\textrm{HD}}\right)$ (i.e., user $i$ is FD and user $\bar{i} \ne i$ is HD), and $\left(\DataRate{}^{\textrm{FD}}/\DataRate{}^{\textrm{HD}}\right)$ (i.e., both users are FD). 


%%
%%
\noindent\textbf{Experimental FD gain}.
For each pair of $(\SNR{1},\SNR{2})$, experimental FD gain is measured in three cases: (i) only user 1 is FD, (ii) only user 2 is FD, and (iii) both users are FD. Fig.~\ref{fig:exp-net-two-users} shows the analytical (colored surface) and experimental (filled circles) FD gain for each case. We exclude the results with $\SNR{i}<\SI{3}{dB}$ since the packets cannot be decoded, resulting in a throughput of zero (see Fig.~\ref{fig:exp-prr-vs-snr}).

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[Only user 1 FD]{
\label{fig:exp-net-two-users-user1-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_user1_fd_gain_experimental.eps}
}
\subfloat[Only user 2 FD]{
\label{fig:exp-net-two-users-user2-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_user2_fd_gain_experimental.eps}
}
\subfloat[Both users FD]{
\label{fig:exp-net-two-users-both-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_both_fd_gain_experimental.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for 3-node networks consisting of one FD BS and two users with varying link SNR values: (a) only user 1 is FD, (b) only user 2 is FD, and (c) both users are FD. The baseline is the network throughput when both users are HD.}
\label{fig:exp-net-two-users}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

%% figure begins
\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{./figs/exp/net_two_users/exp_two_users_fairness.eps}
\vspace{-0.5\baselineskip}
\caption{Measured Jain's fairness index (JFI) in 3-node networks when both users are HD and FD with varying $(\SNR{1},\SNR{2})$.}
\label{fig:exp-net-two-users-fairness}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

The results show that with small link SNR values, the experimental FD gain is lower than the analytical value due to the inability to decode the packets. On the other hand, with sufficient link SNR values, the experimental FD gain exceeds the analytical FD gain. This is because setting $\XINR=1$ in {\eqref{eq:net-two-users-tput-hd-fd}} and {\eqref{eq:net-two-users-tput-fd}} results in a $\SI{3}{dB}$ SNR loss in the analytical FD link SNR, and thereby in a lower throughput. However, in practice, the packets can be decoded with a link PRR of 1 with sufficient link SNRs, resulting in exact twice number of packets being successfully sent over an FD link. Moreover, the FD gain is more significant when enabling FD capability for users with higher link SNR values.

% 0.047/0.036/0.055
Another important metric we consider is the fairness between users, which is measured by the Jain's fairness index (JFI). In the considered 3-node networks, the JFI ranges between 1/2 (worst case) and 1 (best case). Fig.~\ref{fig:exp-net-two-users-fairness} shows the measured JFI when both users operate in HD or FD mode. The results show that introducing FD capability results in an average degradation in the network JFI of only $5.6\%/4.4\%/7.4\%$ for $\SNR{1} = 15/20/25\thinspace\SI{}{dB}$, while the average network FD gains are $1.32\times$/$1.58\times$/$1.73\times$, respectively. In addition, the JFI increases with higher and more balanced user SNR values, which is as expected.


%%%%%
%%%%%
\subsubsection{Heterogeneous 4-Node Networks}
\label{sssec:exp-net-three-users}

We experimentally study 4-node networks consisting of an FD BS and three users with $\SI{10}{dBm}$ TX power (see an example experimental setup in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-three-users}).
% This is limited by the fact that only three FDE PCB cancellers are fabricated, which support one FD BS and at most two FD users.
The experimental setup is similar to that described in Section~\ref{sssec:exp-net-two-users}. 100 experiments are conducts where the 3 users are placed at different locations with different user SNR values. For each experiment, the network throughput is measured in three cases where: (i) zero, (ii) one, and (iii) two users are FD-capable.

Fig.~\ref{fig:exp-net-three-users} shows the CDF of the network throughput of the three cases, where the measured link SNR varies between $5$--$\SI{45}{dB}$. Overall, median network FD gains of $1.25\times$ and $1.52\times$ are achieved in cases with one and two FD users, respectively. The trend shows that in a real-world environment, the total network throughput increases as more users become FD-capable, and the improvement is more significant with higher user SNR values. Note that we only apply a TDMA scheme and a more advanced MAC layer design has the potential to improve the FD gain in these networks.

%% figure begins
\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{./figs/exp/net_three_users/exp_three_users_gain_experimental.eps}
\vspace{-0.5\baselineskip}
\caption{Experimental network throughput gain for 4-node networks when zero, one, or two users are FD-capable, with $\SI{10}{dBm}$ TX power and varying user locations.}
\label{fig:exp-net-three-users}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:

==> tex/intro_20180805.tex <==
Full-duplex (FD) wireless -- simultaneous transmission and reception on the same frequency channel -- can significantly improve spectrum efficiency at the physical (PHY) layer and provide many other benefits at the higher layers~\cite{sabharwal2014band,krishnaswamy2016spectrum}. The main challenge associated with FD is the extremely strong self-interference (SI) signal that needs to be suppressed, requiring $90$-$\SI{110}{dB}$ of self-interference cancellation (SIC). 

% However, as the transmitted signal is many orders of magnitude stronger than the useful signal at the input of the receiver, it is extremely challenging to recover the useful signal and enable such a communication. In particular, the self-interfering (SI) signal needs to be suppressed by billions of times, requiring $90$-$\SI{110}{dB}$ of self-interference cancellation (SIC). 

%%
\begin{figure}[!t]
\centering
\subfloat[]{
\label{fig:intro-pcb}
\includegraphics[height=1.18in]{./figs/testbed/testbed_fde_canc.pdf}}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:intro-fd-radio}
\includegraphics[height=1.18in]{./figs/testbed/testbed_fd_radio.pdf}}
\\ \vspace{-.75\baselineskip}
\subfloat[]{
\label{fig:intro-fd-link}
\includegraphics[width=0.85\columnwidth]{./figs/testbed/testbed_fd_link.png}}
\vspace{-\baselineskip}
\caption{(a) Our frequency-domain equalization- (FDE-) based wideband RF canceller implemented using discrete components on a PCB, (b) our implemented FDE-based FD radio, and (c) \memoTC{replace figure by a network.}}
\label{fig:intro}
\vspace{-\baselineskip}
\end{figure}
%%

Recent work leveraging off-the-shelf components and software-defined radios (SDRs) has established the feasibility of FD wireless through SI suppression at the antenna interface, and SIC in analog/RF and digital domains~\cite{choi2010achieving,duarte2010full,khojastepour2011case,bharadia2013full,korpi2016full}. However, existing approaches to achieve wideband RF SIC (e.g.,~\cite{bharadia2013full, korpi2016full}) rely on RF cancellers with transmission-line delays. Such delay lines cannot be realized in small-form-factor devices and/or integrated circuit (IC) implementations, due to the required lengthy for generating nanosecond-scale time delays and the lossy nature of the silicon substrate.\footnote{For instance, obtaining a nanosecond delay in silicon typically requires a $\SI{15}{cm}$-long delay line.}

A \emph{compact IC-based} design is necessary for supporting FD in hand-held devices (e.g., handsets and tablets). Recently, the first IC-based implementations of wideband FD transceivers have emerged~\cite{yang2015wideband,Zhou_WBSIC_JSSC15}. Recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the technique of frequency-domain equalization (FDE)~\cite{Zhou_WBSIC_JSSC15}. In contrast to the delay line-based approaches (which are essentially performing time-domain equalization), the FDE-based RF canceller utilizes tunable, reconfigurable, high quality factor $2^{\textrm{nd}}$-order bandpass filters (BPFs) with amplitude and phase controls to emulate the frequency-selective antenna interface. In general, tunable, high quality factor BPFs are perhaps as hard to be implemented on an IC as nanosecond-scale delay lines, but $N$-path filters represent an exciting advance that has enabled their implementation in nanoscale CMOS over the past few years~\cite{ghaffari2011tunable,reiskarimian2016analysis}.

% recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the frequency-domain equalization (FDE) of the antenna interface using widely tunable, high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% In contrast to the delay line-based approaches (which are essentially performing time-domain equalization), recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the frequency-domain equalization (FDE) of the antenna interface using widely tunable, high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}.

While major advances have been made at the IC level, there is still a need to understand the fundamental limits of the achievable RF SIC based on technique of FDE and to develop optimized configuration for this new type of RF canceller to achieve optimal RF SIC. It is also important to to evaluate the performance of such compact FD radios in different network settings in real-world environment. \emph{The focus on this paper is on the implementation, optimization, and experimentation of the FDE-based RF canceller that is suitable for wideband compact FD nodes}.
 

% The fundamental challenge associated with achieving wideband RF SIC is due to the frequency selectivity of the antenna interface. Although there has been extensive bench-top implementations of FD transceivers supporting practical levels of SIC across sufficient bandwidth (see ~\cite{bharadia2013full, korpi2016full} and the references in~\cite{sabharwal2014band}), the underlying approaches to achieve SIC at RF (referred to as \emph{RF SIC}) suffer from large radio dimensions that are unsuitable for compact/small-form-factor devices (e.g., laptops and cell phones).

% These approaches to achieve wideband RF SIC are based on transmission-line delays, which are fundamentally impractical to be realized in small-form-factor devices and/or Integrated Circuit (IC) implementations. This is due to the lengthy and bulky transmission-lines required for generating nanosecond-scale true time delays and the lossy nature of the silicon substrate.

% In~\cite{fd_demo_mobihoc16}, we demonstrated an FD radio implementation using a conventional frequency-flat amplitude- and phase-based RF canceller that emulates its RFIC canceller counterpart presented in~\cite{Zhou_NCSIC_JSSC14}. However, this conventional RF canceller can only emulate the antenna interface response at a single frequency point, resulting in a narrowband RF SIC.

% Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}. This new approach is based on frequency-domain equalization (FDE) of the antenna interface using reconfigurable RF bandpass filters (BPFs).
% our work focuses on the design and implementation of wideband compact RF cancellers. Our approach is based on the frequency-domain equalization (FDE) of the antenna interface using reconfigurable RF bandpass filters (BPFs). Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}. In general, tunable, high quality factor filters are perhaps as hard to be implemented on an IC as nanosecond-scale delay lines, but N-path filters represent an exciting advance that has enabled their implementation over the past few years~\cite{ghaffari2011tunable,reiskarimian2016analysis}. Recent advances in the RFIC community have demonstrated the practicality to realize widely tunable high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% Therefore, an RF canceller consisting of multiple FDE taps (BPFs) can channelize the signal bandwidth and emulate the antenna interface. However, there is a lack in both the optimal configuration of the FDE-based canceller and the system-level FD gain introduced by it. \emph{The focus on this paper is on the modeling, optimization, and experimentation of FDE-based wideband RF cancellers that are suitable for compact implementations}.
 
Since while interfacing an RFIC canceller to an SDR presents numerous technical challenges, in this work, we design and implement the FDE-based RF canceller using discrete components on a printed circuit board (PCB), see Fig.~\ref{fig:intro}\subref{fig:intro-pcb} (we refer to it as the \emph{PCB canceller}). The FDE-based PCB canceller can largely facilitate the evaluation of the canceller configuration scheme and the experiments using an SDR platform, as well as to build a network with multiple FDE-based FD nodes.
% In this work, we design and implement the FDE-based RF canceller using discrete components on a printed circuit board (PCB), see Fig.~\ref{fig:intro}\subref{fig:intro-pcb} (we refer to it as the \emph{PCB canceller}).
Moreover, the PCB canceller is more robust and stable to be integrated with the open-access ORBIT~\cite{orbit} and COSMOS~\cite{COSMOS} testbeds to allow the broader community to experiment with wideband compact FD wireless, as we plan to do.\footnote{A narrowband RF canceller has been integrated with the ORBIT testbed~\cite{flexicon_orbit_gen1}.} We present a realistic model of the PCB canceller and its configuration scheme based on an optimization problem. The PCB canceller model is experimentally validated based on measurements and is shown to have high accuracy.

% We present a generalized model for an FDE-based RF canceller and consider two specific models: (i) an \emph{ideal FDE-based canceller} model using $2^{\textrm{nd}}$-order RF BPFs that accurately captures the characteristics of the RFIC canceller~\cite{Zhou_WBSIC_JSSC15}, and (ii) a \emph{FDE-based PCB canceller} model based on an FDE-based RF canceller implemented on a printed circuit board (PCB) in this work. % Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio}and~\ref{fig:intro}\subref{fig:intro-pcb} depict our implemented FD radio equipped with an PCB-based FDE RF canceller that emulates its RFIC counterpart in~\cite{Zhou_WBSIC_JSSC15}, and Fig.~\ref{fig:intro}\subref{fig:intro-fd-link} shows an FD wireless link that we demonstrated in~\cite{fd_demo_infocom17}.
% Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-pcb} depict our implemented FD radio equipped with an PCB-based FDE RF canceller implemented using discrete components.

% The PCB canceller also supports higher TX power handling when compared to the RFIC canceller.

% In order to obtain good RF SIC performance using FDE-based cancellers, we formulate optimization problems with practical constraints for the specific models. In all cases, the objective is to use the FDE-based cancellers to best emulate the antenna interface. Although the non-convex and non-linear nature of the problems results in analytical intractability, we show that the optimization problems can still be numerically solved efficiently. Moreover, in practice, it is unnecessary to find the globally optimal canceller configuration as long as the obtained optimized solution can provide sufficient amount of wideband RF SIC. We also show that when the FDE-based canceller is configured using the solutions to these optimization problems, it performs better than when configured using the iterative configuration algorithm proposed in~\cite{Zhou_WBSIC_JSSC15}.

% We then experimentally validate the PCB canceller model and use them for performance evaluation with the optimized canceller configuration. In particular, the RFIC canceller is numerically evaluated in cases with and without practical hardware constraints. Furthermore, the trade-offs between the RF SIC performance (e.g., desired RF SIC bandwidth) and various configuration parameters (e.g., number of FDE taps) are evaluated. Numerical results show that even under practical constraints, an RFIC canceller with 4 FDE taps is capable of achieving an average $\SI{50}{dB}$ RF SIC across up to $\SI{80}{MHz}$ bandwidth.

We implement an FDE-based FD radio by integrating the PCB canceller with an NI USRP SDR platform, as depicted in Fig.~\ref{fig:intro}\subref{fig:intro-fd-radio}. We experimentally evaluate the performance of the FDE-based FD radio with the canceller configuration scheme, which allows efficient tuning of the PCB canceller to adapt to environmental changes. The FDE-based FD radio achieves $\SI{95}{dB}$ overall SIC across $\SI{20}{MHz}$ real-time bandwidth, enabling an FD link budget of $\SI{10}{dBm}$ average TX power level and $-\SI{85}{dBm}$ RX noise floor. In particular, $\SI{52}{dB}$ SIC is achieved in the RF domain, from which $\SI{20}{dB}$ is obtained from the antenna interface isolation.

We also evaluate the performance and robustness of the FDE-based FD radio at the link-level in the context of packet reception ratio (PRR) and FD throughput gain, in both line-of-sight (LOS) and non-line-of-sight (NLOS) settings. The results show that the FDE-based FD radio achieves an average FD link throughput gain of 1.85$\times$--1.91$\times$, while the link SNR difference when the radio operates in HD and FD modes is only less than $\SI{1}{dB}$.
\memoTC{also add 1(c) of the network}

We extensively evaluate the network-level FD gain in two types of networks, and compare to and confirm the analytical results: (i) \emph{UL-DL networks} consisting of one FD base station (BS) and two half-duplex (HD) users with inter-user interference (IUI), and (ii) \emph{heterogeneous HD-FD networks} consisting of one FD BS and co-existing HD and FD users. For UL-DL networks, we show experimentally that the throughput gain is between  1.14$\times$--1.25$\times$ compared to 1.22$\times$--1.3$\times$ predicted by analysis. We discuss the relationship with UL and DL SNR values, as well as the IUI levels. For heterogeneous HD-FD networks, we demonstrate through experiments the impact of different user SNR values on the throughout, as well as the relationship between the network throughput gain and the number of FD users in the network. For example, in a 4-node network consisting of one FD BS and 3 users with various user locations and SNR values, median experimental FD gains of 1.25$\times$ and 1.52$\times$ can be achieved when one and two users become FD-capable, respectively. To the best of our knowledge, this is the first experimental study of FD gains in such networks. The results can serve as the fundamental building blocks for developing more advanced and efficient MAC layers. The results also demonstrate the performance of compact FD radio designs suitable for hand-held devices, which can be realized through the FDE-based approach.

Finally, we perform sensitivity analysis of the FDE-based cancellers with varying design parameters, and compare the performance between the RFIC and PCB implementations. We show that  optimized canceller configuration is shown to outperform the heuristic canceller configuration in the RFIC implementation~\cite{Zhou_WBSIC_JSSC15} by an order of magnitude in terms of the achieved RF SIC;

%%
%% Contributions
% To summarize, the main contributions of the paper are three-fold:
% \begin{enumerate}[topsep=0pt,itemsep=0pt]%[topsep=0pt, leftmargin=*]
% \item[(i)]
% We present a general FDE-based RF canceller model for achieving wideband RF SIC in compact devices. In addition, two specific models are considered and validated based on our practical implementations of an RFIC canceller and a PCB canceller;
% \item[(ii)]
% We propose an optimization framework for efficiently obtaining optimized FDE-based canceller configuration and use it for performance evaluation of the FDE-based cancellers;
% \item[(iii)]
% We numerically evaluate the RFIC canceller model and the trade-offs between various design parameters. We experimentally evaluate the PCB canceller using an SDR testbed.
% \end{enumerate}

To summarize, the main contributions of the paper are:
\begin{enumerate}[topsep=0pt,itemsep=-5pt]%[topsep=0pt, leftmargin=*]
\item[(i)]
We present the design, implementation, modeling validation, and a canceller configuration scheme of the FDE-based PCB canceller, which can be used to evaluate the performance of FDE-based approach suitable for achieving wideband RF SIC compact nodes;
\item[(ii)]
We experimentally evaluate our FDE-based FD radio with the PCB canceller and the optimized canceller configuration. 
\item[(iii)]
We experimentally evaluate the throughput gain introduced by FD in various network settings with different user capabilities (i.e., HD or FD) and user SNR values.\memoTC{also say something about the sensitivity analysis that we analyze and evaluate the fundamentals for the FDE-based approach?}
\end{enumerate}

The rest of the paper is organized as follows. Section~\ref{sec:related} reviews related work. In Section~\ref{sec:background}, we introduce FD background and the problem formulation, as well as RF canceller designs. We present the design, implementation, and model of the FDE-based PCB canceller, as well as the optimal canceller configuration scheme in Section~\ref{sec:impl}. The performance of the FDE-based FD radio is experimentally evaluated at the node, link, and network levels in Sections~\ref{sec:exp}. In Section~\ref{sec:sensitivity}, we perform sensitivity analysis of the FDE-based cancellers and compare the RFIC and PCB implementations. We conclude and discuss future directions in Section~\ref{sec:conclusion}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:

